Diagnosing applications' I/O behavior through system call observability

We present DIO, a generic tool for observing inefficient and erroneous I/O interactions between applications and in-kernel storage systems that lead to performance, dependability, and correctness issues. DIO facilitates the analysis and enables near real-time visualization of complex I/O patterns for data-intensive applications generating millions of storage requests. This is achieved by non-intrusively intercepting system calls, enriching collected data with relevant context, and providing timely analysis and visualization for traced events. We demonstrate its usefulness by analyzing two production-level applications. Results show that DIO enables diagnosing resource contention in multi-threaded I/O that leads to high tail latency and erroneous file accesses that cause data loss.

==> Makefile <==
TEX = pdflatex -shell-escape -interaction=nonstopmode -file-line-error
PRE =  $(TEX) -ini -job-name="preamble" "&pdflatex preamble.tex\dump"
BIB = bibtex

.PHONY: all view

all : dio.pdf

view :
	open dio.pdf

dio.pdf : dio.tex  dio.bbl dio.blg
	$(TEX) dio.tex
	$(TEX) dio.tex


dio.bbl dio.blg : dio.bib dio.aux
	$(BIB) dio

dio.aux : dio.tex
	$(TEX) dio.tex

dio.bib : dio.tex
	$(TEX) dio.tex

clean:
	rm -f dio.aux dio.bbl dio.blg dio.log dio.out

clean_all:
	rm -f dio.aux dio.bbl dio.blg dio.log dio.out dio.pdf
